Scaling hypothesis for the Euclidean bipartite matching problem

We propose a simple yet very predictive form, based on a Poisson's equation, for the functional dependence of the cost from the density of points in the Euclidean bipartite matching problem. This leads, for quadratic costs, to the analytic prediction of the large $N$ limit of the average cost in dimension $d=1,2$ and of the subleading correction in higher dimension. A non-trivial scaling exponent, $\gamma_d=\frac{d-2}{d}$, which differs from the monopartite's one, is found for the subleading correction. We argue that the same scaling holds true for a generic cost exponent in dimension $d>2$.

==> fig-d1.tex <==
\begin{figure}[h]\pgfplotsset{scaled x ticks=false}
\begin{tikzpicture}[scale=1]
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/.cd,fixed,precision=3},legend pos=north east,legend style={draw=none},
width=0.6\textwidth,height=5cm,xlabel=$N^{-1}$,ylabel=$\frac{1}{N}\beta_N$,yticklabel style={                     /pgf/number format/precision=3},title={Simulations for $d=1$ and $p=2$},domain=0:0.03125,samples=200]
\pgfplotstableread{Enu2d1.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\addplot[black,thick]{0.166668-0.164713*x+0.099099*x^2};
\legend{Numerical data,Fit by $f^{(2)}_1(N)$}
\end{axis}
\end{tikzpicture}\hspace{0.05\textwidth}
\begin{tikzpicture}[scale=1]
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/fixed},legend style={draw=none},
width=0.25\textwidth,height=5cm,xlabel=$N^{-1}$,ylabel=$\beta_N-\frac{N}{6}$,yticklabel style={                     /pgf/number format/precision=3},title={$d=1$},domain=0:0.03125,samples=200]
\pgfplotstableread{Enu2d1bis.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick,dashed]{-0.1645};
\end{axis}
\end{tikzpicture}
\caption{Numerical simulations for $d=1$. We fitted our numerical data for $\frac{1}{N}\bn(1)$ using the three parameters fit function $f^{(2)}_1(N)=\alpha^{(2)}_1+\frac{e_1^{(2)}}{N}+\frac{c}{N^2}$.}
\label{fig:d1}
\end{figure}


==> fig-d2.tex <==

\begin{figure}[h]
\begin{tikzpicture}[scale=1]
\begin{semilogxaxis}[xmax=1,legend pos=south west,legend style={draw=none},
width=0.55\textwidth,height=5cm,xlabel=$N^{-1}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=2$ and $p=2$},domain=0.000025:1,samples=200]
\pgfplotstableread{Enu2d2.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\addplot[black,thick]{-0.1593*ln(x)+0.131225-0.0167666*x^(1/2)};
\legend{Numerical data,Fit by $f^{(2)}_2(N)$}
\end{semilogxaxis}
\end{tikzpicture}\hspace{0.05\textwidth}\pgfplotsset{scaled y ticks=false}\pgfplotsset{scaled x ticks=false}
\begin{tikzpicture}[scale=1]
\begin{semilogxaxis}[xticklabel style={/pgf/number format/fixed,/pgf/number format/precision=3},yticklabel style={/pgf/number format/fixed},legend style={draw=none},width=0.3\textwidth,height=5cm,xlabel=$N^{-1}$,ylabel=$\beta_N-\frac{\ln N}{2\pi}$,yticklabel style={/pgf/number format/precision=3},title={$d=2$},samples=200,domain=0.000025:0.0625]
\pgfplotstableread{Enu2d2bis.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\addplot[black,thick]{0.133225+0.0170451/ln(x)};
%\addplot[black]{0.131225-0.0167666*sqrt(x)};
%\pgfplotstableread{Enu2d2tris.dat}\datatable
%\addplot[only marks,fill=white, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\end{semilogxaxis}
\end{tikzpicture}\caption{Numerical simulations for $d=2$. We fitted our numerical data for $\bn(2)$ using the function $f^{(2)}_2(N)=a\ln N+e_2^{(2)}+\frac{b}{\ln{N}}$. The $\frac{1}{\ln{N}}$ correction was suggested by the right hand plot.}
\label{fig:d2}
\end{figure}


==> fig-d345.tex <==

\begin{figure}[h]
\begin{tikzpicture}[scale=1]
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/fixed},legend style={draw=none},
height=6cm,width=\textwidth,xlabel=$N^{-\gamma_3}$,ylabel=$\beta_N$,yticklabel style={                     /pgf/number format/precision=3},title={Simulations for $d=3$ and $p=2$},domain=0:0.125,samples=200,xtick={0.,0.025,...,0.150}]
\pgfplotstableread{Enu2d3.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\addplot[black,thick]{0.66256-0.448907*x-0.179602*x^3};
\legend{Numerical data,Fit by $f^{(2)}_3(N)$}
\end{axis}\end{tikzpicture}\\\pgfplotsset{scaled x ticks=false, max space between ticks=45pt}\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=3},legend style={draw=none},
height=6cm,width=0.5\textwidth,xlabel=$N^{-\gamma_4}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=4$ and $p=2$},domain=0:0.028,samples=200]
\pgfplotstableread{Enu2d4.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\addplot[black,thick]{0.571294-0.282134*x-0.0110875*x^2};
\legend{Numerical data,Fit by $f^{(2)}_4(N)$}
\end{axis}\end{tikzpicture}\pgfplotsset{max space between ticks=45pt}\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=3},legend style={draw=none},
height=6cm,width=0.5\textwidth,xlabel=$N^{-\gamma_5}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=5$ and $p=2$},domain=0:0.015625,samples=200]
\pgfplotstableread{Enu2d5.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\addplot[black,thick]{0.584785-0.213893*x-0.0289409*x^(5/3)};
\legend{Numerical data,Fit by $f^{(2)}_5(N)$}
\end{axis}
\end{tikzpicture}
\caption{Numerical simulations for $d>2$. We fitted our numerical data for $\bn(d)$ using the function $f^{(2)}_d(N)=e^{(2)}_d+\alpha^{(2)}_d N^{-\gamma_d}+\frac{c}{N}$. The expected value for $\alpha^{(2)}_d$ was $\frac{1}{2\pi^2}\zeta_d(1)$.}
\label{fig:d345}
\end{figure}

==> fig-nu1.tex <==
\begin{figure}[h]
\centering
\iffalse\pgfplotsset{scaled x ticks=false, max space between ticks=45pt}
\begin{tikzpicture}[scale=1]
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=3},legend style={draw=none},
height=6cm,width=\textwidth,xlabel=$N^{-\gamma_3}$,ylabel=$\beta_N$,yticklabel style={                     /pgf/number format/precision=3},title={Simulations for $d=3$},domain=0:0.1666666667,samples=200]
\pgfplotstableread{Enu1d3.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu2d3.dat}\datatable
\addplot[only marks,mark=triangle*, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\pgfplotstableread{Enu3d3.dat}\datatable
\addplot[color=black, fill=white,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu4d3.dat}\datatable
\addplot[mark=square*,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.747214-0.233131*x+0.186038*x^3};
\addplot[black,thick,dashdotted]{0.66256-0.448907*x-0.179602*x^3};
\addplot[black,thick,dashed]{0.631325-0.652189*x+0.277921*x^3};
\addplot[black,thick,dotted]{0.628633-0.86269*x+0.862636*x^3};
\legend{$p=1$,$p=2$,$p=3$,$p=4$}%,$0.74747(4)-0.2380(4)N^{-{1\over 3}}$}
\end{axis}\end{tikzpicture}\\\fi
\pgfplotsset{scaled x ticks=false, max space between ticks=45pt}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=4},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_3}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=3$ and $p=1$},domain=0:0.1428571429,samples=200]
\pgfplotstableread{Enu1d3.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.747214-0.2333131*x-0.186038*x^3};
\legend{$p=1$}
\end{axis}\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=4},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_3}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=3$ and $p=3$},domain=0:0.1666666667,samples=200]
\pgfplotstableread{Enu3d3.dat}\datatable
\addplot[color=black, fill=white,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.631325-0.652189*x+0.277921*x^3};
\legend{$p=3$}
\end{axis}\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=4},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_3}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=3$ and $p=4$},domain=0:0.1666666667,samples=200]
\pgfplotstableread{Enu4d3.dat}\datatable
\addplot[mark=square*,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.628633-0.86269*x+0.862636*x^3};
\legend{$p=4$}
\end{axis}\end{tikzpicture}\\
\pgfplotsset{scaled x ticks=false, max space between ticks=45pt}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=4},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_4}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=4$ and $p=1$},domain=0:0.0277777778,samples=200]
\pgfplotstableread{Enu1d4.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.718145-0.152313*x-0.161782*x^2};
\legend{$p=1$}
\end{axis}\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=4},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_4}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=4$ and $p=3$},domain=0:0.0277777778,samples=200]
\pgfplotstableread{Enu3d4.dat}\datatable
\addplot[color=black, fill=white,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.480354-0.355438*x-0.560822*x^2};
\legend{$p=3$}
\end{axis}\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=4},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_4}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=4$ and $p=4$},domain=0:0.04,samples=200]
\pgfplotstableread{Enu4d4.dat}\datatable
\addplot[mark=square*,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.418285-0.436013*x+0.0138783*x^2};
\legend{$p=4$}
\end{axis}\end{tikzpicture}\\
\pgfplotsset{scaled x ticks=false, max space between ticks=45pt}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=4},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_5}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=5$ and $p=1$},domain=0:0.015625,samples=200]
\pgfplotstableread{Enu1d5.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.739053-0.127297*x+0.063098*x^(5/3)};
\legend{$p=1$}
\end{axis}\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=6},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_5}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=5$ and $p=3$},domain=0:0.015625,samples=200]
\pgfplotstableread{Enu3d5.dat}\datatable
\addplot[color=black, fill=white,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick,dashed]{0.483008-0.275421*x-0.162561*x^(5/3)};
\legend{$p=3$}
\end{axis}\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=6},legend style={draw=none},
height=6cm,width=0.3\textwidth,xlabel=$N^{-\gamma_5}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=5$ and $p=4$},domain=0:0.015625,samples=200]
\pgfplotstableread{Enu4d5.dat}\datatable
\addplot[mark=square*,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.410433-0.344873*x+0.3339*x^(5/3)};
\legend{$p=4$}
\end{axis}\end{tikzpicture}\iffalse\\
\pgfplotsset{max space between ticks=45pt}\begin{tikzpicture}
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=3},legend style={draw=none},
height=6cm,width=0.5\textwidth,xlabel=$N^{-{3\over 5}}$,ylabel=$\beta_N$,yticklabel style={/pgf/number format/precision=3},title={Simulations for $d=5$},domain=0:0.008,samples=200]
\pgfplotstableread{Enu1d5bis.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu2d5bis.dat}\datatable
\addplot[only marks,mark=triangle*, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\pgfplotstableread{Enu3d5.dat}\datatable
\addplot[color=black, fill=white,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu4d5.dat}\datatable
\addplot[mark=square*,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.739038-0.122512*x};
\addplot[black,thick,dashdotted]{0.584785-0.213893*x-0.0289409*x^(5/3)};
\addplot[black,thick,dashed]{0.483019-0.283004*x};
\addplot[black,thick,dotted]{0.410399-0.327219*x};
\legend{$p=1$,$p=2$,$p=3$,$p=4$}
\end{axis}
\end{tikzpicture}\fi
\caption{Numerical simulations for $d>2$. We fitted our numerical data for $\bnu(d)$ using the function $f_{d}^{(p)}(N)=e_d^{(p)}+\alpha_d^{(p)} N^{-\gamma_d}+\frac{c}{N}$. We plotted the results obtained for $p=1,3,4$. Fit results are presented in Table~\ref{tab:nu1}.}
\label{fig:nu1}
\end{figure}

==> fig-nu1old.tex <==
\begin{figure}[h]
\centering

\pgfplotsset{scaled x ticks=false, max space between ticks=45pt}
\begin{tikzpicture}[scale=1]
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=3},legend style={draw=none},
height=6cm,width=\textwidth,xlabel=$N^{-\gamma_3}$,ylabel=$\beta_N$,yticklabel style={                     /pgf/number format/precision=3},title={Simulations for $d=3$},domain=0:0.1666666667,samples=200]
\pgfplotstableread{Enu1d3.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu2d3.dat}\datatable
\addplot[only marks,mark=triangle*, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\pgfplotstableread{Enu3d3.dat}\datatable
\addplot[color=black, fill=white,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu4d3.dat}\datatable
\addplot[mark=square*,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.747214-0.233131*x+0.186038*x^3};
\addplot[black,thick,dashdotted]{0.66256-0.448907*x-0.179602*x^3};
\addplot[black,thick,dashed]{0.631325-0.652189*x+0.277921*x^3};
\addplot[black,thick,dotted]{0.628633-0.86269*x+0.862636*x^3};
\legend{$\nu=1$,$\nu=2$,$\nu=3$,$\nu=4$}%,$0.74747(4)-0.2380(4)N^{-{1\over 3}}$}
\end{axis}\end{tikzpicture}\\
\begin{tikzpicture}[scale=1]
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=3},legend style={draw=none},
height=6cm,width=0.45\textwidth,xlabel=$N^{-\gamma_4}$,ylabel=$\beta_N$,yticklabel style={                     /pgf/number format/precision=3},title={Simulations for $d=4$},domain=0:0.04,samples=200]
\pgfplotstableread{Enu1d4.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu2d4.dat}\datatable
\addplot[only marks,mark=triangle*, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\pgfplotstableread{Enu3d4.dat}\datatable
\addplot[color=black, fill=white,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu4d4.dat}\datatable
\addplot[mark=square*,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.718145-0.152313*x-0.161782*x^2};
\addplot[black,thick,dashdotted]{0.571294-0.282134*x-0.0110875*x^2};
\addplot[black,thick]{0.480354-0.355438*x-0.560822*x^2};
\addplot[black,thick,dotted]{0.418285-0.436013*x+0.0138783*x^2};
\legend{$\nu=1$,$\nu=2$,$\nu=3$,$\nu=4$}%,$0.74747(4)-0.2380(4)N^{-{1\over 3}}$}
\end{axis}\end{tikzpicture}
\begin{tikzpicture}[scale=1]
\begin{axis}[xmin=0,xticklabel style={/pgf/number format/precision=3},legend style={draw=none},
height=6cm,width=0.45\textwidth,xlabel=$N^{-\gamma_5}$,ylabel=$\beta_N$,yticklabel style={                     /pgf/number format/precision=3},title={Simulations for $d=5$},domain=0:0.015625,samples=200]
\pgfplotstableread{Enu1d5.dat}\datatable
\addplot[only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu2d5.dat}\datatable
\addplot[only marks,mark=triangle*, error bars/.cd,y dir=both,y explicit] table[y=E, y error=dE] from \datatable;
\pgfplotstableread{Enu3d5.dat}\datatable
\addplot[color=black, fill=white,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\pgfplotstableread{Enu4d5.dat}\datatable
\addplot[mark=square*,only marks, error bars/.cd,y dir=both,y explicit] table[y=y, y error=dy] from \datatable;
\addplot[black,thick]{0.739053-0.127297*x+0.063098*x^(5/3)};
\addplot[black,thick,dashdotted]{0.584785-0.213893*x-0.0289409*x^(5/3)};
\addplot[black,thick,dashed]{0.483008-0.275421*x-0.162561*x^(5/3)};
\addplot[black,thick]{0.410433-0.344873*x+0.3339*x^(5/3)};
\legend{$p=1$,$p=2$,$p=3$,$p=4$}%,$0.74747(4)-0.2380(4)N^{-{1\over 3}}$}
\end{axis}\end{tikzpicture}

\caption{Numerical simulations for $d>2$. We fitted our numerical data for $\bnu(d)$ using the function $f_{d}^{(p)}(N)=e_d^{(p)}+\alpha_d^{(p)} N^{-\gamma_d}+\frac{c}{N}$. We plotted the results obtained for $p=1,3,4$. Fit results are presented in Table~\ref{tab:nu1}.}
\label{fig:nu1}
\end{figure}
